Beta-VAE Reproducibility: Challenges and Extensions

$\beta$-VAE is a follow-up technique to variational autoencoders that proposes special weighting of the KL divergence term in the VAE loss to obtain disentangled representations. Unsupervised learning is known to be brittle even on toy datasets and a meaningful, mathematically precise definition of disentanglement remains difficult to find. Here we investigate the original $\beta$-VAE paper and add evidence to the results previously obtained indicating its lack of reproducibility. We also further expand the experimentation of the models and include further more complex datasets in the analysis. We also implement an FID scoring metric for the $\beta$-VAE model and conclude a qualitative analysis of the results obtained. We end with a brief discussion on possible future investigations that can be conducted to add more robustness to the claims.

==> preamble.tex <==
%\documentclass[11pt, oneside, paper=A4, DIV=15, BCOR=0mm, abstract=true]{scrartcl}
\usepackage[english]{babel}
%\documentclass{article}    sorry can be changed back if you want
%\usepackage[utf8]{inputenc}
\usepackage{mathtools}
\usepackage{amssymb}
\usepackage{rawfonts}
\usepackage{oldlfont}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage[headsepline, automark]{scrlayer-scrpage}
\usepackage{physics}
\usepackage{tabularx}
\usepackage{verbatim}

\usepackage{titlesec}
\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
\renewcommand{\thesubsubsection}{\thesubsection.\arabic{subsubsection}}

\titleformat{\section}{\centering \bfseries}{\thesection.}{0.5em}{}
\titleformat{\subsection}[runin]{\bfseries}{\normalfont\thesubsection.}{0.5em}{}
\titleformat{\subsubsection}[runin]{\it}{\thesubsubsection.}{0.5em}{}
\titlespacing{\section}{0pt}{2.0ex plus .5ex
     minus .2ex}{1.0ex plus .2ex}
     
     
     
%table of contents
\usepackage{titletoc}
\titlecontents{section}[1.5em]{}{\contentslabel{1.5em}}{\hspace*{-1.5em}}{\titlerule*[8pt]{.}\contentspage}



%header and footer
\pagestyle{scrheadings}

\clearscrheadfoot
%\ohead{  \ifstr{\rightbotmark}{\leftmark}{}{\rightbotmark}}
\ihead{whatever }
\rohead*{\leftmark}
%\ihead{Candidate Number: }
%\ohead{Abschlussbericht}
%\ifoot{Gruppe 1 -- Biogas}
\setlength{\footskip}{50pt}
\cfoot{- \pagemark \ -}
